LogiDebrief: A Signal-Temporal Logic based Automated Debriefing Approach with Large Language Models Integration

Emergency response services are critical to public safety, with 9-1-1 call-takers playing a key role in ensuring timely and effective emergency operations. To ensure call-taking performance consistency, quality assurance is implemented to evaluate and refine call-takers' skillsets. However, traditional human-led evaluations struggle with high call volumes, leading to low coverage and delayed assessments. We introduce LogiDebrief, an AI-driven framework that automates traditional 9-1-1 call debriefing by integrating Signal-Temporal Logic (STL) with Large Language Models (LLMs) for fully-covered rigorous performance evaluation. LogiDebrief formalizes call-taking requirements as logical specifications, enabling systematic assessment of 9-1-1 calls against procedural guidelines. It employs a three-step verification process: (1) contextual understanding to identify responder types, incident classifications, and critical conditions; (2) STL-based runtime checking with LLM integration to ensure compliance; and (3) automated aggregation of results into quality assurance reports. Beyond its technical contributions, LogiDebrief has demonstrated real-world impact. Successfully deployed at Metro Nashville Department of Emergency Communications, it has assisted in debriefing 1,701 real-world calls, saving 311.85 hours of active engagement. Empirical evaluation with real-world data confirms its accuracy, while a case study and extensive user study highlight its effectiveness in enhancing call-taking performance.

==> 8_ack.tex <==
\section*{Acknowledgment}
This work was supported in part by the U.S. National Science Foundation under Grants \todo{add references here}, the Google Academic Research Award, OpenAI Researcher Access Program, and the U.S. Department of Education under Grant R305C240010. The opinions, findings, conclusions, or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the sponsoring agencies.

\noindent \todo{\textbf{Stakeholder Discussion} The development of \textit{LogiDebrief} was grounded in a close, iterative collaboration with the Metro Nashville Department of Emergency Communications (MNDEC). Their domain expertise directly shaped the system’s design, from surfacing critical quality assurance gaps to co-specifying over 2,200 procedural requirements in formal logic. Beyond problem framing, MNDEC actively participated in refining runtime thresholds, validating output interpretations, and integrating the tool into ongoing training. Beyond the reported 4-week case study, \textit{LogiDebrief} continues to be used as part of MNDEC’s ongoing training and quality assurance workflows. The partnership transitioned from initial prototyping to field deployment, establishing a scalable model for AI-assisted QA that aligns with operational needs and is now being explored for broader regional adoption.}


